Generalized Bradley-Terry Models for Score Estimation from Paired Comparisons

Many applications, e.g. in content recommendation, sports, or recruitment, leverage the comparisons of alternatives to score those alternatives. The classical Bradley-Terry model and its variants have been widely used to do so. The historical model considers binary comparisons (victory or defeat) between alternatives, while more recent developments allow finer comparisons to be taken into account. In this article, we introduce a probabilistic model encompassing a broad variety of paired comparisons that can take discrete or continuous values. We do so by considering a well-behaved subset of the exponential family, which we call the family of generalized Bradley-Terry (GBT) models, as it includes the classical Bradley-Terry model and many of its variants. Remarkably, we prove that all GBT models are guaranteed to yield a strictly convex negative log-likelihood. Moreover, assuming a Gaussian prior on alternatives' scores, we prove that the maximum a posteriori (MAP) of GBT models, whose existence, uniqueness and fast computation are thus guaranteed, varies monotonically with respect to comparisons (the more A beats B, the better the score of A) and is Lipschitz-resilient with respect to each new comparison (a single new comparison can only have a bounded effect on all the estimated scores). These desirable properties make GBT models appealing for practical use. We illustrate some features of GBT models on simulations.

==> acknowledgment.tex <==
\section*{Acknowledgments}
\label{sec:acknowledgements}

We are indebted to the tens of thousands contributors who compared videos, 
developed our code base, promoted the Tournesol platform
and donated to the Tournesol Association.

\len{Deadline: February 6. 14 pages max. \url{https://facctconference.org/2023/cfp.html}}



==> app-mle.tex <==
Justification for the regularization. ToDo.

        \begin{proposition} \label{prop:nonresilient}
    We fix a GBT model such that $\Dc$ is bounded. Then, the MLE $\Theta^*(\Comp)$ is not $\beta$-resilient for any $\beta > 0$.        
    \end{proposition}


        \begin{proof}[Proof of {prop:nonresilient}]
        The boundedness of $\Dc$ implies that $\Ds = \R$. 
        We  consider the case where only one comparison $r_{ab} = r$ is performed, for which we estimate two scores $\theta_a,\theta_b$ such that $\theta_a + \theta_b = 0$. It is equivalent to estimated $\theta = \theta_{ab} = \theta_a - \theta_b = 2 \theta_a$. 
        The GBT estimator is the unique solution to
        \begin{equation}
            \theta^*(r) = \arg \min_{\theta \in \R} \quad \Phi(\theta) - r\theta,
        \end{equation}
        which is characterized by $\partial_\theta \mathcal{L}(\theta^*(r)|r) = \Phi'(\theta^*(r)) - r = 0$, or equivalently 
        \begin{equation}
        \theta^*(r) = (\Phi')^{-1} (r) .   
        \end{equation}
        The latter is valid since we know from Theorem~\ref{theo:Phi} that $\Phi'$ is a continuous strictly increasing bijection from $\Ds=\R$ to its image $\Phi'(\Ds) = \Dc$. This means in particular that $\theta^*(r) = (\Phi')^{-1} (r) \rightarrow_{r\rightarrow 1} \infty$, hence one can arbitrarily modify the $\theta^*(r)$ by changing $r$. This implies that $\theta^*(r)$ is not $\beta$-resilient for any $\beta > 0$. 
    \end{proof}

    
